Video Coding with Cross-Component Sample Offset

Beyond the exploration of traditional spatial, temporal and subjective visual signal redundancy in image and video compression, recent research has focused on leveraging cross-color component redundancy to enhance coding efficiency. Cross-component coding approaches are motivated by the statistical correlations among different color components, such as those in the Y'CbCr color space, where luma (Y) color component typically exhibits finer details than chroma (Cb/Cr) color components. Inspired by previous cross-component coding algorithms, this paper introduces a novel in-loop filtering approach named Cross-Component Sample Offset (CCSO). CCSO utilizes co-located and neighboring luma samples to generate correction signals for both luma and chroma reconstructed samples. It is a multiplication-free, non-linear mapping process implemented using a look-up-table. The input to the mapping is a group of reconstructed luma samples, and the output is an offset value applied on the center luma or co-located chroma sample. Experimental results demonstrate that the proposed CCSO can be applied to both image and video coding, resulting in improved coding efficiency and visual quality. The method has been adopted into an experimental next-generation video codec beyond AV1 developed by the Alliance for Open Media (AOMedia), achieving significant objective coding gains up to 3.5\,\% and 1.8\,\% for PSNR and VMAF quality metrics, respectively, under random access configuration. Additionally, CCSO notably improves the subjective visual quality.

==> tables/bo_and_eo_on_lumachroma.tex <==
\begin{tabular}{cccccccccc}%{c|c|c|c|c|c}
    \bottomrule
                      &            & Y         & U         & V         & YUV       & VMAF      & Enc-time & Dec-time \\
    \bottomrule
    \multirow{6}*{AI} & A1$\_$4k   & -0.52\,\% & 0.10\,\%  & 0.11\,\%  & -0.45\,\% & -0.81\,\% & 115\,\%  & 113\,\%  \\
    \cline{2-9}
                      & A2$\_$2k   & -0.36\,\% & 0.12\,\%  & 0.13\,\%  & -0.32\,\% & -0.77\,\% & 109\,\%  & 110\,\%  \\
    \cline{2-9}
                      & A3$\_$720p & -0.39\,\% & 0.15\,\%  & 0.14\,\%  & -0.34\,\% & -0.52\,\% & 108\,\%  & 109\,\%  \\
    \cline{2-9}
                      & A4$\_$360p & -0.43\,\% & 0.17\,\%  & 0.18\,\%  & -0.38\,\% & -0.62\,\% & 106\,\%  & 104\,\%  \\
    \cline{2-9}
                      & A5$\_$270p & -0.09\,\% & 0.28\,\%  & 0.29\,\%  & -0.06\,\% & -0.36,\%  & 106\,\%  & 101\,\%  \\
    \cline{2-9}
                      & B1$\_$SYN  & -0.42\,\% & 0.09\,\%  & 0.09\,\%  & -0.37\,\% & -0.59\,\% & 107\,\%  & 107\,\%  \\
    \cline{2-9}
                      & AVG        & -0.39\,\% & 0.13\,\%  & 0.13\,\%  & -0.34\,\% & -0.66\,\% & 108\,\%  & 109\,\%  \\
    \bottomrule

    \multirow{6}*{RA} & A1$\_$4k   & -0.76\,\% & 0.07\,\%  & 0.21\,\%  & -0.69\,\% & -1.82\,\% & 113\,\%  & 117\,\%  \\
    \cline{2-9}
                      & A2$\_$2k   & -0.41\,\% & 0.07\,\%  & 0.08\,\%  & -0.37\,\% & -1.14\,\% & 107\,\%  & 110\,\%  \\
    \cline{2-9}
                      & A3$\_$720p & -0.29\,\% & 0.07\,\%  & 0.05\,\%  & -0.25\,\% & -0.82\,\% & 108\,\%  & 110\,\%  \\
    \cline{2-9}
                      & A4$\_$360p & -0.32\,\% & 0.17\,\%  & 1.20\,\%  & -0.25\,\% & -0.41\,\% & 106\,\%  & 108\,\%  \\
    \cline{2-9}
                      & A5$\_$270p & 0.05\,\%  & 0.21\,\%  & 0.50\,\%  & 0.08\,\%  & -0.62,\%  & 106\,\%  & 106\,\%  \\
    \cline{2-9}
                      & B1$\_$SYN  & -0.54\,\% & -0.17\,\% & 0.30\,\%  & -0.48\,\% & -1.18\,\% & 106\,\%  & 106\,\%  \\
    \cline{2-9}
                      & AVG        & -0.43\,\% & 0.04\,\%  & 0.28\,\%  & -0.37\,\% & -1.09\,\% & 108\,\%  & 110\,\%  \\
    \bottomrule

    \multirow{6}*{LD} & A1$\_$4k   & -         & -         & -         & -         & -         & -        & -        \\
    \cline{2-9}
                      & A2$\_$2k   & -0.61\,\% & 0.13\,\%  & 0.37\,\%  & -0.54\,\% & -0.72\,\% & 106\,\%  & 110\,\%  \\
    \cline{2-9}
                      & A3$\_$720p & -0.56\,\% & -0.03\,\% & 0.08\,\%  & -0.50\,\% & -0.89\,\% & 108\,\%  & 109\,\%  \\
    \cline{2-9}
                      & A4$\_$360p & -0.36\,\% & 0.05\,\%  & -0.41\,\% & -0.35\,\% & 0.12\,\%  & 107\,\%  & 109\,\%  \\
    \cline{2-9}
                      & A5$\_$270p & -0.12\,\% & 0.71\,\%  & -0.60\,\% & -0.09\,\% & -0.50\,\% & 106\,\%  & 105\,\%  \\
    \cline{2-9}
                      & B1$\_$SYN  & -0.59\,\% & 0.25\,\%  & -0.26\,\% & -0.53\,\% & -0.83\,\% & 106\,\%  & 106\,\%  \\
    \cline{2-9}
                      & AVG        & -0.53\,\% & 0.17\,\%  & 0.02\,\%  & -0.47\,\% & -0.66\,\% & 106\,\%  & 109\,\%  \\
    \bottomrule
\end{tabular}

==> tables/bo_only.tex <==
\begin{tabular}{cccccccccc}%{c|c|c|c|c|c}
  \bottomrule
                    &            & Y         & U         & V         & YUV       & VMAF      & Enc-time & Dec-time \\
  \bottomrule
  \multirow{6}*{AI} & A1$\_$4k   & 0.09\,\%  & -1.45\,\% & -1.62\,\% & -0.12\,\% & 0.11\,\%  & 105\,\%  & 101\,\%  \\
  \cline{2-9}
                    & A2$\_$2k   & 0.07\,\%  & -1.85\,\% & -1.70\,\% & -0.10\,\% & 0.08\,\%  & 102\,\%  & 101\,\%  \\
  \cline{2-9}
                    & A3$\_$720p & 0.04\,\%  & -1.07\,\% & -0.87\,\% & -0.04\,\% & 0.05\,\%  & 101\,\%  & 98\,\%   \\
  \cline{2-9}
                    & A4$\_$360p & 0.06\,\%  & -1.53\,\% & -0.47\,\% & -0.03\,\% & 0.06\,\%  & 102\,\%  & 95\,\%   \\
  \cline{2-9}
                    & A5$\_$270p & 0.06\,\%  & -0.29\,\% & -0.12\,\% & 0.04\,\%  & 0.06\,\%  & 102\,\%  & 96\,\%   \\
  \cline{2-9}
                    & B1$\_$SYN  & 0.05\,\%  & -0.76\,\% & -0.82\,\% & -0.04\,\% & 0.06\,\%  & 102\,\%  & 101\,\%  \\
  \cline{2-9}
                    & AVG        & 0.06\,\%  & -1.34\,\% & -1.17\,\% & -0.07\,\% & 0.07\,\%  & 102\,\%  & 100\,\%  \\
  \bottomrule

  \multirow{6}*{RA} & A1$\_$4k   & -0.17\,\% & -1.82\,\% & -2.01\,\% & -0.37\,\% & -0.33\,\% & 103\,\%  & 100\,\%  \\
  \cline{2-9}
                    & A2$\_$2k   & 0.02\,\%  & -2.32\,\% & -1.46\,\% & -0.14\,\% & 0.01\,\%  & 101\,\%  & 100\,\%  \\
  \cline{2-9}
                    & A3$\_$720p & 0.04\,\%  & -2.11\,\% & -0.97\,\% & -0.10\,\% & -0.05\,\% & 102\,\%  & 103\,\%  \\
  \cline{2-9}
                    & A4$\_$360p & 0.03\,\%  & -2.41\,\% & -0.90\,\% & -0.11\,\% & 0.04\,\%  & 102\,\%  & 97\,\%   \\
  \cline{2-9}
                    & A5$\_$270p & 0.04\,\%  & -0.32\,\% & -0.40\,\% & 0.01\,\%  & 0.11\,\%  & 100\,\%  & 97\,\%   \\
  \cline{2-9}
                    & B1$\_$SYN  & 0.03\,\%  & -1.04\,\% & -1.18\,\% & -0.08\,\% & 0.12\,\%  & 102\,\%  & 101\,\%  \\
  \cline{2-9}
                    & AVG        & 0.00\,\%  & -1.84\,\% & -1.29\,\% & -0.14\,\% & -0.01\,\% & 101\,\%  & 100\,\%  \\
  \bottomrule

  \multirow{6}*{LD} & A1$\_$4k   & -         & -         & -         & -         & -         & -        & -        \\
  \cline{2-9}
                    & A2$\_$2k   & 0.06\,\%  & -2.56\,\% & -1.65\,\% & -0.12\,\% & 0.00\,\%  & 101\,\%  & 100\,\%  \\
  \cline{2-9}
                    & A3$\_$720p & 0.03\,\%  & -2.20\,\% & -1.07\,\% & -0.12\,\% & 0.00\,\%  & 101\,\%  & 98\,\%   \\
  \cline{2-9}
                    & A4$\_$360p & 0.10\,\%  & -2.71\,\% & -0.92\,\% & -0.05\,\% & -0.01\,\% & 101\,\%  & 101\,\%  \\
  \cline{2-9}
                    & A5$\_$270p & 0.05\,\%  & -1.00\,\% & -1.12\,\% & -0.04\,\% & 0.00\,\%  & 101\,\%  & 102\,\%  \\
  \cline{2-9}
                    & B1$\_$SYN  & 0.03\,\%  & -0.98\,\% & -1.87\,\% & -0.10\,\% & 0.07\,\%  & 102\,\%  & 100\,\%  \\
  \cline{2-9}
                    & AVG        & 0.05\,\%  & -2.04\,\% & -1.49\,\% & -0.10\,\% & 0.01\,\%  & 101\,\%  & 100\,\%  \\
  \bottomrule
\end{tabular}

==> tables/edge_clf_type.tex <==
\begin{tabular}{cccccccccc}%{c|c|c|c|c|c}
  \bottomrule
                    &            & Y         & U         & V          & YUV       & VMAF      & Enc-time & Dec-time \\
  \bottomrule
  \multirow{6}*{AI} & A1$\_$4k   & 0.10\,\%  & -3.51\,\% & -3.64\,\%  & -0.33\,\% & 0.13\,\%  & 102\,\%  & 106\,\%  \\
  \cline{2-9}
                    & A2$\_$2k   & 0.06\,\%  & -3.15\,\% & -4.09\,\%  & -0.28\,\% & 0.09\,\%  & 102\,\%  & 102\,\%  \\
  \cline{2-9}
                    & A3$\_$720p & 0.05\,\%  & -3.45\,\% & -2.47\,\%  & -0.23\,\% & 0.06\,\%  & 102\,\%  & 98\,\%   \\
  \cline{2-9}
                    & A4$\_$360p & 0.08\,\%  & -6.76\,\% & -9.40\,\%  & -0.58\,\% & 0.09\,\%  & 102\,\%  & 98\,\%   \\
  \cline{2-9}
                    & A5$\_$270p & 0.10\,\%  & -4.37\,\% & -2.55\,\%  & -0.21\,\% & 0.11\,\%  & 100\,\%  & 97\,\%   \\
  \cline{2-9}
                    & B1$\_$SYN  & 0.03\,\%  & -2.58\,\% & -2.63\,\%  & -0.18\,\% & 0.05\,\%  & 101\,\%  & 101\,\%  \\
  \cline{2-9}
                    & AVG        & 0.06\,\%  & -3.57\,\% & -3.95\,\%  & -0.28\,\% & 0.08\,\%  & 101\,\%  & 101\,\%  \\
  \bottomrule

  \multirow{6}*{RA} & A1$\_$4k   & 0.21\,\%  & -7.37\,\% & -9.09\,\%  & -0.73\,\% & 0.25\,\%  & 100\,\%  & 112\,\%  \\
  \cline{2-9}
                    & A2$\_$2k   & 0.13\,\%  & -6.64\,\% & -8.25\,\%  & -0.54\,\% & 0.15\,\%  & 100\,\%  & 114\,\%  \\
  \cline{2-9}
                    & A3$\_$720p & 0.09\,\%  & -4.67\,\% & -4.44\,\%  & -0.33\,\% & 0.16\,\%  & 101\,\%  & 98\,\%   \\
  \cline{2-9}
                    & A4$\_$360p & 0.17\,\%  & -6.60\,\% & -7.10\,\%  & -0.48\,\% & 0.12\,\%  & 101\,\%  & 98\,\%   \\
  \cline{2-9}
                    & A5$\_$270p & 0.05\,\%  & -6.25\,\% & -1.75\,\%  & -0.31\,\% & -0.32\,\% & 100\,\%  & 107\,\%  \\
  \cline{2-9}
                    & B1$\_$SYN  & 0.04\,\%  & -4.92\,\% & -3.87\,\%  & -0.33\,\% & 0.11\,\%  & 101\,\%  & 100\,\%  \\
  \cline{2-9}
                    & AVG        & 0.12\,\%  & -6.10\,\% & -6.43\,\%  & -0.47\,\% & 0.12\,\%  & 100\,\%  & 106\,\%  \\
  \bottomrule

  \multirow{6}*{LD} & A1$\_$4k   & -         & -         & -          & -         & -         & -        & -        \\
  \cline{2-9}
                    & A2$\_$2k   & 0.04\,\%  & -8.84\,\% & -10.84\,\% & -0.84\,\% & 0.12\,\%  & 100\,\%  & 110\,\%  \\
  \cline{2-9}
                    & A3$\_$720p & 0.12\,\%  & -5.27\,\% & -4.56\,\%  & -0.32\,\% & 0.24\,\%  & 101\,\%  & 97\,\%   \\
  \cline{2-9}
                    & A4$\_$360p & 0.15\,\%  & -7.30\,\% & -7.91\,\%  & -0.56\,\% & 0.18\,\%  & 101\,\%  & 104\,\%  \\
  \cline{2-9}
                    & A5$\_$270p & 0.16\,\%  & -6.89\,\% & -0.62\,\%  & -0.17\,\% & 0.53\,\%  & 100\,\%  & 99\,\%   \\
  \cline{2-9}
                    & B1$\_$SYN  & -0.02\,\% & -7.09\,\% & -5.09\,\%  & -0.52\,\% & 0.04\,\%  & 101\,\%  & 101\,\%  \\
  \cline{2-9}
                    & AVG        & 0.06\,\%  & -7.56\,\% & -7.42\,\%  & -0.60\,\% & 0.16\,\%  & 100\,\%  & 104\,\%  \\
  \bottomrule
\end{tabular}

==> tables/overall.tex <==
\begin{tabular}{cccccccccc}%{c|c|c|c|c|c}
  \bottomrule
                    &            & Y         & U         & V         & YUV       & VMAF     & Enc-time & Dec-time \\
  \bottomrule
  \multirow{6}*{AI} & A1$\_$4k   & 0.11\,\%  & 5.21\,\%  & 4.87\,\%  & 0.67\,\%  & 0.39\,\% & 93\,\%   & 92\,\%   \\
  \cline{2-9}
                    & A2$\_$2k   & 0.16\,\%  & 4.44\,\%  & 6.20\,\%  & 0.60\,\%  & 0.76\,\% & 96\,\%   & 94\,\%   \\
  \cline{2-9}
                    & A3$\_$720p & 0.26\,\%  & 3.01\,\%  & 2.70\,\%  & 0.48\,\%  & 0.53\,\% & 98\,\%   & 95\,\%   \\
  \cline{2-9}
                    & A4$\_$360p & 0.22\,\%  & 6.45\,\%  & 4.51\,\%  & 0.61\,\%  & 0.78\,\% & 99\,\%   & 91\,\%   \\
  \cline{2-9}
                    & A5$\_$270p & 0.04\,\%  & 1.23\,\%  & 0.24\,\%  & 0.10\,\%  & 0.50\,\% & 98\,\%   & 93\,\%   \\
  \cline{2-9}
                    & B1$\_$SYN  & 0.38\,\%  & 2.01\,\%  & 1.84\,\%  & 0.53\,\%  & 0.99\,\% & 96\,\%   & 92\,\%   \\
  \cline{2-9}
                    & B2$\_$SCC  & 0.57\,\%  & 1.69\,\%  & 1.66\,\%  & 0.66\,\%  & 2.03\,\% & 98\,\%   & 96\,\%   \\
  \cline{2-9}
                    & AVG w/o B2 & 0.20\,\%  & 3.92\,\%  & 4.20\,\%  & 0.55\,\%  & 0.70\,\% & 96\,\%   & 93\,\%   \\
  \cline{2-9}
                    & AVG w B2   & 0.26\,\%  & 3.56\,\%  & 3.79\,\%  & 0.56\,\%  & 0.91\,\% & 97\,\%   & 94\,\%   \\
  \bottomrule

  \multirow{6}*{RA} & A1$\_$4k   & 0.34\,\%  & 8.28\,\%  & 6.91\,\%  & 1.10\,\%  & 0.79\,\% & 95\,\%   & 93\,\%   \\
  \cline{2-9}
                    & A2$\_$2k   & 0.20\,\%  & 7.39\,\%  & 9.50\,\%  & 0.82\,\%  & 0.67\,\% & 97\,\%   & 96\,\%   \\
  \cline{2-9}
                    & A3$\_$720p & 0.19\,\%  & 5.46\,\%  & 3.04\,\%  & 0.55\,\%  & 0.49\,\% & 97\,\%   & 97\,\%   \\
  \cline{2-9}
                    & A4$\_$360p & 0.09\,\%  & 9.68\,\%  & 6.09\,\%  & 0.68\,\%  & 0.56\,\% & 99\,\%   & 98\,\%   \\
  \cline{2-9}
                    & A5$\_$270p & -0.23\,\% & 1.00\,\%  & 1.40\,\%  & -0.12\,\% & 0.38\,\% & 98\,\%   & 100\,\%  \\
  \cline{2-9}
                    & B1$\_$SYN  & 0.33\,\%  & 3.55\,\%  & 3.42\,\%  & 0.61\,\%  & 0.93\,\% & 97\,\%   & 96\,\%   \\
  \cline{2-9}
                    & B2$\_$SCC  & 1.13\,\%  & 3.83\,\%  & 3.53\,\%  & 1.36\,\%  & 3.63\,\% & 91\,\%   & 96\,\%   \\
  \cline{2-9}
                    & AVG w/o B2 & 0.20\,\%  & 6.38\,\%  & 6.29\,\%  & 0.70\,\%  & 0.67\,\% & 97\,\%   & 96\,\%   \\
  \cline{2-9}
                    & AVG w B2   & 0.35\,\%  & 5.97\,\%  & 5.85\,\%  & 0.81\,\%  & 1.14\,\% & 96\,\%   & 96\,\%   \\
  \bottomrule

  \multirow{6}*{LD} & A1$\_$4k   & -         & -         & -         & -         & -        & -        & -        \\
  \cline{2-9}
                    & A2$\_$2k   & 0.40\,\%  & 9.45\,\%  & 10.92\,\% & 1.08\,\%  & 0.64\,\% & 97\,\%   & 95\,\%   \\
  \cline{2-9}
                    & A3$\_$720p & 0.16\,\%  & 4.68\,\%  & 4.11\,\%  & 0.51\,\%  & 0.08\,\% & 96\,\%   & 93\,\%   \\
  \cline{2-9}
                    & A4$\_$360p & 0.05\,\%  & 10.46\,\% & 7.79\,\%  & 0.69\,\%  & 0.43\,\% & 98\,\%   & 94\,\%   \\
  \cline{2-9}
                    & A5$\_$270p & -0.12\,\% & 2.81\,\%  & 1.98\,\%  & 0.05\,\%  & 0.10\,\% & 99\,\%   & 94\,\%   \\
  \cline{2-9}
                    & B1$\_$SYN  & 0.44\,\%  & 5.37\,\%  & 3.97\,\%  & 0.79\,\%  & 0.94\,\% & 97\,\%   & 94\,\%   \\
  \cline{2-9}
                    & B2$\_$SCC  & 1.52\,\%  & 4.10\,\%  & 4.21\,\%  & 1.74\,\%  & 3.65\,\% & 92\,\%   & 95\,\%   \\
  \cline{2-9}
                    & AVG w/o B2 & 0.28\,\%  & 7.46\,\%  & 7.35\,\%  & 0.80\,\%  & 0.54\,\% & 97\,\%   & 94\,\%   \\
  \cline{2-9}
                    & AVG w B2   & 0.51\,\%  & 6.85\,\%  & 6.78\,\%  & 0.97\,\%  & 1.10\,\% & 96\,\%   & 94\,\%   \\
  \bottomrule
\end{tabular}

==> tables/overall_gain.tex <==
\begin{tabular}{cccccccccc}%{c|c|c|c|c|c}
    \bottomrule
                      &            & Y         & U         & V         & YUV       & VMAF(Y)     & Enc-time & Dec-time \\
    \bottomrule
    \multirow{6}*{AI} & A1$\_$4k   & -0.11\,\%  & -4.85\,\%  & -4.55\,\%  & -0.66\,\%  & -0.38\,\% & 107\,\%   & 109\,\%   \\
    \cline{2-9}
                      & A2$\_$2k   & -0.16\,\%  & -4.11\,\%  & -5.34\,\%  & -0.59\,\%  & -0.75\,\% & 104\,\%   & 107\,\%   \\
    \cline{2-9}
                      & A3$\_$720p & 0-.25\,\%  & -2.89\,\%  & -2.59\,\%  & -0.48\,\%  & -0.52\,\% & 102\,\%   & 105\,\%   \\
    \cline{2-9}
                      & A4$\_$360p & -0.21\,\%  & -6.03\,\%  & -4.15\,\%  & -0.61\,\%  & -0.77\,\% & 101\,\%   & 109\,\%   \\
    \cline{2-9}
                      & A5$\_$270p & -0.04\,\%  & -1.21\,\%  & -0.24\,\%  & -0.10\,\%  & -0.50\,\% & 102\,\%   & 107\,\%   \\
    \cline{2-9}
                      & B1$\_$SYN  & -0.37\,\%  & -1.94\,\%  & -1.77\,\%  & -0.52\,\%  & -0.98\,\% & 104\,\%   & 107\,\%   \\
    \cline{2-9}
                      & B2$\_$SCC  & -0.56\,\%  & -1.57\,\%  & -1.58\,\%  & -0.65\,\%  & -1.90\,\% & 103\,\%   & 104\,\%   \\
    \cline{2-9}
                      & AVG w/o B2 & -0.20\,\%  & -3.67\,\%  & -3.76\,\%  & -0.54\,\%  & -0.69\,\% & 104\,\%   & 107\,\%   \\
    \cline{2-9}
                      & AVG w B2   & -0.26\,\%  & -3.33\,\%  & 3.41\,\%  & -0.56\,\%  & -0.88\,\% & 104\,\%   & 107\,\%   \\
    \bottomrule
  
    \multirow{6}*{RA} & A1$\_$4k   & -0.33\,\%  & -7.37\,\%  & -6.30\,\%  & -1.08\,\%  & -0.77\,\% & 106\,\%   & 107\,\%   \\
    \cline{2-9}
                      & A2$\_$2k   & -0.20\,\%  & -6.43\,\%  & -7.94\,\%  & -0.80\,\%  & -0.66\,\% & 103\,\%   & 104\,\%   \\
    \cline{2-9}
                      & A3$\_$720p & -0.19\,\%  & -5.00\,\%  & -2.86\,\%  & -0.54\,\%  & -0.48\,\% & 103\,\%   & 103\,\%   \\
    \cline{2-9}
                      & A4$\_$360p & -0.09\,\%  & -8.66\,\%  & -5.20\,\%  & -0.67\,\%  & -0.55\,\% & 101\,\%   & 98\,\%   \\
    \cline{2-9}
                      & A5$\_$270p & 0.23\,\% & -0.97\,\%  & -1.31\,\%  & 0.12\,\% & -0.38\,\% & 102\,\%   & 100\,\%  \\
    \cline{2-9}
                      & B1$\_$SYN  & -0.32\,\%  & -3.34\,\%  & -3.21\,\%  & -0.60\,\%  & -0.91\,\% & 103\,\%   & 104\,\%   \\
    \cline{2-9}
                      & B2$\_$SCC  & -1.11\,\%  & -3.56\,\%  & -3.28\,\%  & -1.33\,\%  & -3.45\,\% & 110\,\%   & 105\,\%   \\
    \cline{2-9}
                      & AVG w/o B2 & -0.20\,\%  & -5.68\,\%  & -5.46\,\%  & -0.69\,\%  & -0.66\,\% & 103\,\%   & 104\,\%   \\
    \cline{2-9}
                      & AVG w B2   & -0.34\,\%  & -5.34\,\%  & -5.11\,\%  & -0.79\,\%  & -1.11\,\% & 104\,\%   & 104\,\%   \\
    \bottomrule
  
    \multirow{6}*{LD} & A1$\_$4k   & -         & -         & -         & -         & -        & -        & -        \\
    \cline{2-9}
                      & A2$\_$2k   & -0.39\,\%  & -7.71\,\%  & -8.88\,\%  & -1.05\,\%  & -0.63\,\% & 104\,\%   & 106\,\%   \\
    \cline{2-9}
                      & A3$\_$720p & -0.16\,\%  & -4.42\,\%  & -3.83\,\%  & -0.51\,\%  & -0.08\,\% & 104\,\%   & 107\,\%   \\
    \cline{2-9}
                      & A4$\_$360p & -0.05\,\%  & -9.21\,\% & -6.74\,\%  & -0.68\,\%  & -0.43\,\% & 102\,\%   & 106\,\%   \\
    \cline{2-9}
                      & A5$\_$270p & 0.12\,\% & -2.57\,\%  & -1.81\,\%  & -0.05\,\%  & -0.09\,\% & 101\,\%   & 106\,\%   \\
    \cline{2-9}
                      & B1$\_$SYN  & -0.43\,\%  & -4.89\,\%  & -3.69\,\%  & -0.78\,\%  & -0.91\,\% & 103\,\%   & 106\,\%   \\
    \cline{2-9}
                      & B2$\_$SCC  & -1.48\,\%  & -3.73\,\%  & -3.86\,\%  & -1.69\,\%  & -3.46\,\% & 109\,\%   & 105\,\%   \\
    \cline{2-9}
                      & AVG w/o B2 & -0.28\,\%  & -6.39\,\%  & -6.21\,\%  & -0.79\,\%  & -0.53\,\% & 103\,\%   & 106\,\%   \\
    \cline{2-9}
                      & AVG w B2   & -0.49\,\%  & -5.91\,\%  & -5.79\,\%  & -0.95\,\%  & -1.06\,\% & 104\,\%   & 106\,\%   \\
    \bottomrule
  \end{tabular}

==> tables/syntax.tex <==
\def \lineh {0.04cm}
\begin{threeparttable}
\begin{tabular}{ll}
  \toprule
  \textbf{Syntax} & \textbf{Descriptor} \\
  \midrule
  frame\_header() \{ & \\[\lineh]
  \ldots & \\[\lineh]
  \textbf{\textit{ccso\_frame\_flag}} & u(1)${}^\ast$ \\[\lineh]
  \ \ if (ccso\_frame\_flag)\{ & \\[\lineh]
  \ \ \ \ for (plane=0; plane$<$num\_planes; plane++ )\{ & \\[\lineh]
  \ \ \ \ \ \textbf{\textit{ccso\_enable}}[plane] & u(1) \\[\lineh]
  \ \ \ \ \ \ \ if( ccso\_enable[plane])\{ & \\[\lineh]
  \ \ \ \ \ \ \ \ \ \textbf{\textit{ccso\_bo\_only}}[plane] & u(1) \\[\lineh]
  \ \ \ \ \ \ \ \ \ if (ccso\_bo\_only[plane])\{ & \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \textbf{\textit{max\_band\_log2}}[plane] & u(3) \\[\lineh]
  \ \ \ \ \ \ \ \ \ \} else \{ & \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \textbf{\textit{max\_band\_log2}}[plane] & u(2) \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \textbf{\textit{quant\_step\_idx}}[plane] & u(2) \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \textbf{\textit{filter\_shape\_idx}}[plane] & u(3) \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \textbf{\textit{edge\_clf}}[plane] & u(1) \\[\lineh]
  \ \ \ \ \ \ \ \ \ \} & \\ [0.1cm]
  \ \ \ \ \ \ \ \ \ max\_band = 1 $\ll$ max\_band\_log2 & \\[\lineh]
  \ \ \ \ \ \ \ \ \ intervals = ccso\_bo\_only ? 1 : (~edge\_clf + 2) & \\[\lineh]
  \ \ \ \ \ \ \ \ \ for (d0=0; d0$<$intervals; d0++)\{ & \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ for (d1=0; d1$<$intervals; d1++)\{ & \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \ \ for (bdn=0; bdn$<$max\_band; bdn++)\{ & \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ ccso\_idx = bnd $\ll$ 4 + d0 $\ll$ 2 + d1 & \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \textbf{\textit{offset\_idx}} & tu${}^\dagger$ \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ offset\_lut[plane][ccso\_idx] & \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ = offsets[offset\_idx]& \\[\lineh]
  \ \ \ \ \ \ \ \ \ \ \ \ \ \} & \\ [0.1cm]
  \ \ \ \ \ \ \ \ \ \ \ \} & \\ [0.1cm]
  \ \ \ \ \ \ \ \ \ \} & \\ [0.1cm]
  \ \ \ \ \ \ \ \} & \\ [0.1cm]
  \ \ \ \ \} & \\ [0.1cm]
  \ \ \} & \\ [0.1cm]
  \ldots & \\[0.1cm]
  \} & \\ [0.1cm]
  \bottomrule
\end{tabular}
\begin{tablenotes}
    \footnotesize
    \item ${}^\ast$ fixed-length coded syntax elements.
    \item ${}^\dagger$ truncated unary coded syntax elements.
  \end{tablenotes}
\end{threeparttable}    
